LaForge: Always-Correct and Fast Incremental Builds from Simple Specifications

Developers rely on build systems to generate software from code. At a minimum, a build system should produce build targets from a clean copy of the code. However, developers rarely work from clean checkouts. Instead, they rebuild software repeatedly, sometimes hundreds of times a day. To keep rebuilds fast, build systems run incrementally, executing commands only when built state cannot be reused. Existing tools like make present users with a tradeoff. Simple build specifications are easy to write, but limit incremental work. More complex build specifications produce faster incremental builds, but writing them is labor-intensive and error-prone. This work shows that no such tradeoff is necessary; build specifications can be both simple and fast. We introduce LaForge, a novel build tool that eliminates the need to specify dependencies or incremental build steps. LaForge builds are easy to specify; developers write a simple script that runs a full build. Even a single command like gcc src/*.c will suffice. LaForge traces the execution of the build and generates a transcript in the TraceIR language. On later builds, LaForge evaluates the TraceIR transcript to detect changes and perform an efficient incremental rebuild that automatically captures all build dependencies. We evaluate LaForge by building 14 software packages, including LLVM and memcached. Our results show that LaForge automatically generates efficient builds from simple build specifications. Full builds with LaForge have a median overhead of 16.1% compared to a project's default full build. LaForge's incremental builds consistently run fewer commands, and most take less than 3.08s longer than manually-specified incremental builds. Finally, LaForge is always correct.

==> algorithms.tex <==
\section{Algorithm}
\label{sec:algorithms}

\riker's build algorithm is modeled as a fixed-point procedure over a build's effects:
the algorithm starts with the current state of the build and performs work until no new effects are produced.
During each iteration, the \riker algorithm looks for changes.
Whenever changes are found, the corresponding command is marked to run.
Before the algorithm is complete, \riker runs all such marked commands.
\riker traces every command executed, and during tracing \traceir is generated.
Whenever rebuild executes a command that has \traceir information available, the old \traceir is replaced.
\riker continues this process until it finds no new changes.
Conveniently, a full build is just a degenerate case of an incremental build.

\riker finds changes by interleaving command emulation with real command execution.
Command emulation is achieved by evaluating \traceir.
The smallest primitive in the \traceir language is a \emph{step}, which is a predicate over system state.
% Evaluation entails a few discrete aspects, which we refer to as \emph{emulation}, \emph{tracing}, and \emph{planning} and discuss in this section.
\riker always evaluates steps in a \emph{model} of system state, which is initially populated with the filesystem's real state.
Whenever the model indicates a change and \riker determines that a command must run, modeled state is written lazily and the command is executed.
% Handling state in this way enables \riker to model an incremental build as if it were a full build, making it easy to guarantee that the effect of running an incremental build is always the same as the effect of running a full build.

\paragraph{Weak equivalance.}
\label{sec:weakequiv}
A core principle at the heart of \riker's build algorithm is \emph{weak equivalence}.
Two artifacts are weakly equivalent if they were produced by two invocations of the same command with the same arguments in the same environment.
Weak equivalence is a stronger guarantee about the equivalence of program outputs than the one provided by \make.
\make targets are assumed to be equivalent given the same input, but that guarantee does not extend to state generated by subcommands.

% Weak equivalence allows \riker to reason about commands that exhibit nondeterminism.
In the presence of nondeterminism, weak equivalence implies that \emph{all} of the possible outputs are \emph{substitutable} for a given input.
% Build tools like \gcc and \clang utilize nondeterminism extensively.
Because this idea pervades \riker's design, \riker can use off-the-shelf build tools that exhibit nondeterminism---like \gcc and \clang---without special logic.

% Weak equivalence implies that when nondeterminism is encountered in a build, \emph{any} of the possible outputs are \emph{equivalent} for a given input.
% \riker aggressively applies this principle to avoid doing unnecessary work, and as a consequence, \riker is able to automatically produce incremental builds not just over the set of commands supplied by the user, but over all commands in the build, including subcommands.
% We extensively evaluate \riker against real-world benchmarks (see~\sectref{sec:evaluation}), and our correctness tests justify this decision.

\subsection{Fixed-point Build Algorithm}
We start by describing \riker algorithm's outermost routine, shown in Figure~\ref{fig:dobuild}.
The purpose of the algorithm is to identify and run the set of commands that must run because of changed inputs.

\paragraph{Definitions.}
$E$ is the \emph{environment}, which maps references to artifact states (see~\sectref{sec:artifacts} for details).
Artifacts roughly correspond to objects in UNIX that can be referred to through \texttt{inode}s.
\emph{Artifact state} refers to either the metadata or contents of an artifact.
An artifact state may be \emph{committed}, which means that it reflects actual system state, or \emph{uncommitted}, which means that it represents modeled state.
Artifact states may also be \emph{cached}, which means that either \riker stores a copy of their contents or it can recreate that state on-demand.
Some artifacts are \emph{uncacheable}.
For example, \riker caches file contents, but not pipe contents.
$R$ is the set of commands that must run.
$T$ is a trace, which is a list of \traceir steps.
$D$ is a graph of \emph{command dependencies}, which maps commands that must run to the set of commands that depend on those commands through artifacts.

\paragraph{Lazy commit model.}
Most of \riker's logic is concerned with maintaining the environment, $E$.
The purpose of $E$ is to model system state, which enables \riker to reason about what commands need to run by comparing $E$ against the actual state of the filesystem.
Effects are learned by emulating a build in the context of $E$, which also updates $E$.
\riker follows a simple rule during emulation:
if a command's effect is different or cannot be determined---because a command has never run before---the command must be \emph{traced}.

Tracing a command means that it is executed in a \ptrace environment that intercepts all syscalls (see~\sectref{sec:implementation} for details).
As all stateful effects in UNIX occur through syscalls, syscall interposition provides a convenient, narrow interface for capturing dependencies.
During tracing, effects are recorded in $E$ and the command's corresponding \traceir predicates are appended to $T$.
% Command effects are unknown in two circumstances: either one of the command's dependencies changed  or the command has never been seen before by \riker.
% In the first case, \riker knows that a command's dependency changed when a modeled change in $E$ does not match actual system state.
% The second case occurs when a trace has no record of having run a command.

% All other commands are \emph{emulated}, meaning that \riker infers their effects and stores them in $E$.
When a command is traced, its effect on state is necessarily reflected as actual system state, which we call \emph{committed state}.
By contrast, emulated commands prefer to keep state \emph{uncommitted}---only visible in $E$---until the moment that the build requires that it manifest as actual system state.
State is committed from $E$ whenever a traced command needs to access it, and at the end of the build when state changes should become visible to the user.
This \emph{lazy commit model} allows \riker to rapidly infer changes while minimizing the amount of system state actually altered.
% This behavior is highly desirable.
% For example, when a user runs a build without changing any files, \riker will determine changes without ever running any commands or changing any system state.

\begin{figure}[t]
	\small
	\begin{center}
	  \begin{codebox}
		\Procname{$\proc{DoBuild}(trpath)$}
		  \li $i \gets 1$
		  \li $E \gets$ \mbox{\{\;\}}
		  \li $R \gets$ \mbox{\{ \}}\label{line:incrbuild}
		  \li $T \gets$ \proc{LoadTrace}($trpath$)\label{line:loadtrace}
		  \li \If $|T| \isequal 0$ \Then
			\li $T \gets$ \mbox{\{ \IRLaunch(\rkr, \rikerfile, ...) \}}\label{line:cleanbuild}
		  \End
		  \li \Repeat \label{line:whilecommands}
			\li $E \gets$ \proc{Sync}($E$)\label{line:sync1}
		  	\li $(E, T, D, R) \gets$ \proc{Emulate}($E$, $T$, \mbox{false})\label{line:emulate1}
			\li $R \gets$ \proc{Plan}($D$, $R$)\label{line:plan}
			\li $i \gets i + 1$
		  \li \Until $|R| > 0$\label{line:whileend}
		  \li \proc{CommitAll}($env$)\label{line:commitall}
		  \li \If $i > 1$ \Then\label{line:post-build}
			\li $(\_, T, \_, \_) \gets$ \proc{Emulate}($E$, $T$, $R$, \mbox{\{\;\}}, \mbox{true})\label{line:emulate2}
		  \End
		  \li \proc{WriteTrace}($T$)\label{line:writetrace}
	  \end{codebox}
	\end{center}
	\caption{
	  \small
	  The outermost routine of \riker's build algorithm.
	  This procedure interleaves emulation and tracing until the build produces no new changes.
	  At the end of the \texttt{while} loop, the build is up-to-date.
	  The final call to \proc{Emulate} captures post-build state.
	  \label{fig:dobuild}
	}
  \end{figure}

\paragraph{First full build.}
When \riker is asked to build a project the first time, it starts only with the user-supplied \rikerfile.
There is no on-disk \traceir trace, $T$, since the build has not run before.
Traces are recorded during a build and are stored by in a local \file{.rkr} directory.
On the first build, \proc{LoadTrace} returns the empty list (Figure~\ref{fig:dobuild}, line~\ref{line:loadtrace}).
To bootstrap the process, \riker populates the initial trace, $R$, with a launch of the user's \rikerfile (line~\ref{line:cleanbuild}).
\riker iterates over a build until the set of commands to run, $R$, is empty (lines~\ref{line:whilecommands}--\ref{line:whileend}).

\proc{Sync} discards all uncommitted state in $E$ (line~\ref{line:sync1}).
During the first iteration, $E$ is empty so there is nothing to discard.

\proc{Emulate}, shown in Figure~\ref{fig:emulate} (line~\ref{line:emulate1}), is responsible for evaluating all of the \traceir steps in $T$.
\proc{Emulate} evaluates \traceir steps in the order that they appear in the given trace, $T$.
We define \proc{Emulate} in Figure~\ref{fig:emulate}.
% \proc{Emulate} strictly only evaluates \traceir steps for commands in the set $R$, except when a command is newly launched by a traced command and therefore has not been encountered before.
Evaluation of a \traceir step essentially checks that conditions in $E$ match actual system state.
For example, if a command expects that a file exists with specific contents, one of that command's steps will compare the contents of the file in $E$ with the actual contents of the file on disk.
Whenever \riker finds a difference, the actual system state has \emph{changed}.
When a change is detected, the associated command is added to $R$.
Whenever a \IRLaunch command is encountered, and the target command is in $R$, the command is traced.
Both evaluation and tracing write traces to a new trace buffer.
When a command is emulated, \riker simply echoes its existing \traceir steps into the buffer.
Tracing a command always replaces its existing steps with a new sequence of steps.
After tracing a given command, it is removed from $R$.

\proc{Eval} launches \traceir-specific evaluation rules(see~\sectref{sec:traceir}); during that process, \riker tracks the set of commands that consume artifacts generated by a traced command.
This information is used to more efficiently plan the next set of commands to run (line~\ref{line:plan}).
For example, if \cmd{cc1} writes to a file \file{tmp.s} which is later read by \cmd{as}, the mapping \cmd{cc1} $\rightarrow$ \texttt{\{} \cmd{as} \texttt{\}} is added to $D$, the \emph{command dependence graph}.
$D$ is returned with the updated environment, $E$, trace, $T$, and set of commands to run, $R$.

On the first iteration of a full build, $T$ contains only the \rikerfile \IRLaunch step, so \proc{Emulate} marks the \rikerfile to run.
On the next iteration, \rikerfile is traced, updating $E$ with all the events it observes while also appending new \traceir predicates to the trace buffer.
Since all of the subcommands launched by the \rikerfile at this point have never been encountered before, they are also traced.
As \proc{Emulate} has no prior trace during a full build, it never observes changes, and therefore $R$ is empty at the end of the first iteration.
\proc{CommitAll} (line~\ref{line:commitall}), which ensures that all emulated effects are materialized in the filesystem, does nothing in the first full build because all commands are emulated.

Line~\ref{line:post-build} ensures that a \emph{post-build check} is carried out after a build is done, except when a build does nothing.
The purpose of a post-build check is to augment $T$ with extra predicates that short-circuit a build when the build's state on disk already matches its intended final state.
For example, if a build contains the command \cmd{cat a > b}, it does not need to re-run if \file{a} is unchanged and \texttt{b} already exists.
Finally, \proc{WriteTrace} stores the new trace to disk for use during the next call to \rkr.
At the end of the \proc{DoBuild} routine, all commands given in the user's \rikerfile have run, and all effects are visible on disk, meaning that the project has been built.

\begin{figure}[t]
	\small
	\begin{center}
	  \begin{codebox}
		\Procname{$\proc{Emulate}(E, T, R, post)$}
		\li $T' \gets$ \mbox{nil} % stores the new trace
		\li $D \gets$ \mbox{\{\;\}} % stores command -> { command }, the set of command deps
		\li $R' =$ \mbox{\{\;\}}
		\li \For $t$ \kw{in} $T$ \Do
			\li $c \gets \CmdOf{t}$
			\li \If $c \notin R$ \Then
				% NOTE: D only contains the commands whose outputs we cannot commit
				\li $(ts, E, D, same) \gets \Eval{t}{E}{R}{D}{post}$ \label{line:eval}
				\li \If $\lnot same$ \Then
					\li $R' \gets R' \cup \{ c \}$
				\End
				\li $T' \gets T' \mbox{@} \; ts$
			\End
	    \End
	    \li \Return ($E$, $T'$, $D$, $R'$)
	  \end{codebox}
	\end{center}
	\caption{
	  \small
	  \proc{Emulate} evaluates the effect of \traceir steps from emulated or traced commands.
	  Traced commands (those in $R$) are always launched by calling \proc{Eval} on a \IRLaunch predicate (line\ref{line:eval}).
	  $T'$ is a new, initially empty, trace buffer.
	  $D$ is the command dependence graph, which stores which commands must run when other commands run.  
	  \proc{Eval} takes a \traceir step ($t$), the environment ($E$), the current command dependence graph ($D$), and a boolean that states whether pre-build or post-build predicates should be emitted.
	  \proc{Eval} returns a new trace fragment ($ts$), updated environment ($E$), updated command dependence graph ($D$), and a boolean flag that says whether the predicate observed a change ($same$).
	  $T$ and $ts$ are linked lists, and \mbox{@} is the list append operator.
	  \label{fig:emulate}
	}
  \end{figure}

\paragraph{Incremental build.}
An incremental build occurs when \rkr starts with an existing trace.
% In this scenario, the user makes zero or more changes to artifacts involved in the build.
% Any observable alteration to system state can be a change: it could be a change to a project source file, a change to a project directory, including the addition or removal of files, a change to file or directory metadata, the alteration of any binary executable used in the build toolchain, as well as any change to the system kernel itself that manifests as a change to syscall semantics.
As in a full build, \proc{Emulate} begins with $E$ initially empty.
Again, at the start of an incremental build, $R$ is empty because the role of the first iteration is to find commands to run by checking \traceir predicates.
Although there are some subtleties (see~\sectref{sec:planning} and~\sectref{sec:skipping}), as a general rule, \traceir evaluation always leads
 \riker to conclude that a command either \emph{must run} or \emph{is skippable}.
In the former case, the command is added to $R$; in the latter case, evaluation of a command's \traceir updates $E$ with uncommitted state.
Whenever \IRLaunch is encountered for a command already in $R$, the command is traced.
\riker always completely evaluates $T$ during a call to \proc{Emulate}.

\proc{Plan} computes the set of all commands reachable through dependence edges in order to find groups of commands that must run concurrently.
We describe \proc{Plan} in detail in~\sectref{sec:planning}.



\subsection{Build Planning}
\label{sec:planning}

The purpose of the \proc{Plan} procedure is to find \emph{command clusters}.
A command cluster is a strongly connected component~\cite{DBLP:journals/siamcomp/Tarjan72} of a dependency graph that contains only command vertices.
This graph is induced by linking commands to each other through dependencies.
%The commands \cmd{collect2} and \cmd{ld} in Figure~\ref{fig:example} are a command cluster.
%\cmd{collect2} starts \cmd{ld} which takes in object files and outputs \file{program} and two output streams;
%\cmd{ld}'s \file{stdout} and \file{stderr} streams are redirected to files which are read by \cmd{collect2}.
%\cmd{collect2} and \cmd{ld} are a command cluster because they are strongly connected through dependency edges.
%This arrangement enables \cmd{collect2} to re-run \cmd{ld} with different flags depending after an initial link attempt.
%Command clusters prevent na\"ive incremental build algorithms from terminating.
\riker uses an approach inspired by the well-known mark-sweep algorithm~\cite{10.1145/367177.367199} to ensure that commands in a cluster always run together.

The essential problem with command clusters is that of dependence cycles.
% Without considering potential cycles, \proc{DoBuild} only detects a change for one party at a time for a given loop iteration.
To illustrate, suppose \cmd{A} and \cmd{B} are a command cluster.
Initially, neither \cmd{A} nor \cmd{B} are marked to run, but on the first iteration, \cmd{A} observes an input change.
In the second iteration, \riker traces \cmd{A}, emulating \cmd{B} and detecting a change for \cmd{B}.
\cmd{B} is marked to run.
In the third iteration, \riker traces \cmd{B}, emulating \cmd{A} and detecting a change for \cmd{B}.
\cmd{A} is marked to run.
Without corrective action, the build algorithm will loop indefinitely.

\riker circumvents this problem for file and directory artifacts, by ensuring that their emulated state can be committed (i.e., restored) on demand, allowing one or more commands in a cluster to be replayed during emulation.
\riker currently does not cache states for pipe or socket contents, so any commands that read from the same pipe will form a command cluster that must run together.
We leave caching for these types to future work.

% \proc{Proc} has additional performance benefits, because it eagerly marks commands that should clearly run without having to wait until the next iteration emulates them.
% For example, referring to the motivating example in Figure~\ref{fig:example}, if \cmd{cc1} runs and produces a new object file, \proc{Plan} will eagerly mark \cmd{as} to run so that it is traced in the next loop iteration.

\paragraph{Marking and mark propagation rules.}
\proc{Plan} takes the command dependence graph, $D$, and the set of changed commands, $R$, as its input.
Marking starts with commands in $R$.
$R$ functions similarly to ``object roots'' from garbage collection literature.
\proc{Plan} follows all edges in the command dependence graph, propagating the initial markings (i.e., adding commands to the set $R$).
While $D$ could be computed in the \proc{Plan} procedure, for efficiency reasons, $D$ is instead constructed during \traceir step evaluation.
Commands are added to $D$ during evaluation whenever the following mark propagation rules hold.

\textbf{Definitions.}
Let $c$ be a command.
By convention, $c_1$ to refers to a command that produces an output and $c_2$ to refers to a command that consumes that output.
Let $P_c$ be the set of predicates associated with command $c$.
Let $s$ be an artifact state.
Let $R$ be the set of commands that must run.
Let $E$ be the environment.
Let $\Sigma$ be the set of cached artifact states.
Let \Inputs{$c$} be the set of artifact states read by command $c$, and let \Outputs{$c$} be the set of artifact states written by command $c$.

\begin{enumerate}[leftmargin=0cm,itemindent=.5cm,labelwidth=\itemindent,labelsep=1em,align=left,label=(\arabic*) , wide=0pt, font=\itshape]
	% Rule 1 in the code.
	\item $\exists p \in P_c, \lnot p(c) \implies c \in R$ \label{rule:1} \\
	If $c$ has at least one failed predicate, $c$ must run.
	This rule is a direct consequence of the principle of weak equivalence (see~\sectref{sec:weakequiv}).
	\riker can only reason about effects for commands that have been observed for given inputs.

	% Rule 2 in the code.
	\item $\exists s \in \Outputs{c}, s \in E \land s \notin \Sigma \implies c \in R$ \label{rule:2} \\
	If a command writes to an artifact, and that artifact's state persists in the environment but is not cached, the command that produced it must always run. 
	This rule simulates \make targets.
	In other words, files left over at the end of the build should be reproduced when the build reruns.

	% Rule 3 in the code.
	\item $c_2 \in R \land (\exists s \in \Outputs{c_1}, s \in \Inputs{c_2} \land s \notin \Sigma) \implies c_1 \in R$\label{rule:3}\\
	If a command $c_1$ writes an artifact that is not cached that another command $c_2$ consumes, and $c_2$ is marked to run, $c_1$ must run. 
	This rule is distinct from rule~\ref{rule:2} because these artifacts need not persist in the environment.
	This rule ensures that if, for example, a producer communicates with a consumer that is marked to run, the producer is also marked to run.

	% Rule 5 in the code.
	\item $c_1 \in R \land (\exists s \in \Outputs{c_1}, s \in \Inputs{c_2} \land s \notin \Sigma) \implies c_2 \in R$\label{rule:4}\\
	If a command $c_2$ reads an artifact that is not cached that another command $c_1$ produces, and $c_1$ is marked to run, $c_2$ must run.
	This rule is similar to rule~\ref{rule:3}, except that it refers to the consumer instead of the producer.

	% We omit rules 6 and 7 which produce MayRun markings that we no longer use.
	% We also omit rules 4 and 8 which are "run once" optimizations.

\end{enumerate}

\subsection{Command Skipping}
\label{sec:skipping}

Build commands often launch subcommands, but in an incremental build not all of those subcommands need to run.
In our motivating example (see~\sectref{sec:overview}), a file is added to the build. 
The incremental build runs the \rikerfile because \riker detects a change in the \IRCWD.
Because the shell expands the wildcard, \file{*.c}, into an additional file, \file{z.c}, \riker detects a change and runs \gcc.
The two source files, \file{x.c} and \file{y.c}, did not change and do not need to be rebuilt, so \cmd{cc1} for both commands can be skipped.
% \riker skips commands, emulating them instead, if the previous emulation and planning iteration did not mark them to rerun.
% The command skipping mechanism makes it possible to produce incremental builds from simple build specifications like the one in the example.

\riker matches command invocations using a \emph{command invocation template}.
This template includes the name of the function and its command-line arguments.
However, temporary file name arguments introduce a complication: file names are often random.
To address this, \riker considers any file artifact that appears in \file{/tmp} to be a temporary file.
Additionally, if a child command accesses tempfile content in a previous build, then that tempfile content for candidates commands must also match.
With this handling, \riker can recognize that a new command invocation is actually the same as a previous invocation modulo tempfile names.
% This last requirement is to prevent spurious matches, which improves performance.
% Although matching incorrectly does not affect correctness, bad matches unnecessarily report changes and trigger rebuilds.

The order that \riker emulates commands in the presence of command skipping exploits a set of ordering relations~\cite{10.1145/3335772.3335934} observed during the previous build.
As long as emulation preserves this order, the build is guaranteed to correctly produce a weakly-equivalent build.
From the viewpoint of the parent process of a potentially skipped command, all of the child's actions are potentially visible at the moment the parent command issues an \syscall{exec} call to launch the child command.

In our example, \riker knows that \cmd{cc1} is potentially skippable because it was not marked for execution.
When \cmd{cc1} is launched, \riker searches for a matching template.
If no match is found, \riker lets \gcc launch \cmd{cc1} as usual.
If a match is found, \riker suspends \gcc and immediately evaluates \cmd{cc1}'s trace.
\riker then resumes \gcc.
A dummy process with the appropriate register state ensures that when \gcc \syscall{wait()}s for \cmd{cc1}, the emulated \cmd{cc1}'s exit code is returned.
If \gcc needs to read inputs written by \cmd{cc1}, such artifacts are lazily committed on demand.

% DWB: we don't have space for this:
% A keen observer might object that, in the scenario above, after \gcc launches \cmd{cc1}, if \gcc were to write outputs that \cmd{cc1} was supposed to read, the emulated \cmd{cc1} in this scenario will not observe them.
% Fortunately, when these events transpire, \cmd{cc1}'s emulation will detect a change.
% If the difference in the files matters---if a happens-before edge should exist between \gcc's write and \cmd{cc1}'s read---\riker will mark \cmd{cc1} to run in the next iteration, emulating \gcc and tracing \cmd{cc1}.
% If the difference doesn't matter, then the build can freely interleave events between \gcc and \cmd{cc1}.
% In fact, this handling is in keeping with \riker's weak equivalence guarantee: \emph{any} product of a nondeterministic build is acceptable, including potentially racy ones, because the build \emph{could have} produced that sequence of events.

% DWB: again, no room
% Candidate templates are generated in the order that a trace is processed.
% Since child commands are guaranteed to have been emulated before \riker needs to decide whether to launch or skip a child command, the set of candidate templates will always include a match if there is one.


\subsection{Exit Code Changes}
\label{sec:exitcodechanges}

Ideally, \riker executes commands that need to be run at most once.
Unfortunately, exit codes introduce a wrinkle that means that \riker cannot always guarantee single executions.
For example, when a programmer mistakenly introduces bugs that produce compile-time errors---an extremely common occurrence---command exit codes will change.
When a traced child command that produces a changed exit code is returned to an emulated parent command, the parent command's behavior may also change.
\riker addresses this problem by rerunning the parent command.


==> redis-case-study.tex <==
\redis is a high-performance key-value store implemented in approximately 80,000 source lines of C code~\cite{redis}.
We evaluate \riker against \redis' included \Makefile.
We omit the \rikerfile used to build \redis for space reasons, but it resembles the \rikerfile for \cmd{xz}.
% One key difference is that \redis uses many \file{.c} files in multiple target programs (as opposed to just four for \cmd{xz}).
% Our \rikerfile for \redis compiles all \file{.c} files once before passing them to the remaining build commands.
% This adds one line to the \rikerfile, but the change is intuitive, aligns with the behavior of \redis' included \Makefile, and results in significantly shorter compile times.

% \todo[inline]{Put the complete \rikerfile is in the appendix}

An interesting element of \redis' build system is that it generates a \file{release.h} file to encode the current \cmd{git} revision.
The provided build system includes extra checks to avoid touching the generated file when the \cmd{git} revision has not changed, since \make interprets updated \texttt{mtime}s as changed dependencies.
Our \rikerfile generates the same file, but does not need extra logic.
\riker traces the \cmd{git} command that produces the revision ID and runs it again only when \cmd{git}'s internal state is updated.

\begin{figure}[t]
  \begin{center}
    \includegraphics{graphs/redis}
    \caption{
      Command counts and runtimes for 100 incremental builds of \redis.
      \riker runs 51\% fewer commands than \make.
      \riker's builds take $2.13\times$ longer than \make, but just $1.45\times$ for builds that run at least 10\% of commands.
      \label{fig:redis}
    }
  \end{center}
\end{figure}

Figure~\ref{fig:redis} shows \redis build results.
% As with \cmd{xz}, the version of \redis built by \riker passes all included tests.
The \riker build runs 51\% fewer commands than \make, and takes $2.13\times$ longer on average.
\riker's trace is 22.9MB, and its cache contains 174 files totaling 80.1MB.
\riker's runtime overhead is clearly distorted by \riker's longer builds for small numbers of commands;
when the build runs at least 10\% of the number of commands from the full build \riker's overhead is just $1.5\times$.

\riker's overhead for this benchmark is attributed to a few causes.
When a command is suspended on a syscall stop during tracing \riker generates new \traceir steps, evaluates these steps, and serializes them to an on-disk buffer for the next phase.
At the same time, \riker does its fingerprinting and caching of files.
Of these tasks, only the generation and evaluation of \traceir needs to happen before the command can be resumed;
other tasks could be offloaded for background processing.
We plan to implement this change and expect that it will reduce \riker's overhead significantly, particularly for short-lived commands that touch many files like the \cmd{git} command mentioned earlier.
As Figure~\ref{fig:redis} shows, \make also suffers high overheads for this case.
Nevertheless, \riker is almost always able to update incremental builds in less time than a full build.

%\begin{figure}[t]
%  \begin{center}
%    \includegraphics{graphs/redis.count}
%    \caption{
%      The number of times a subset of commands executed while building \cmd{redis}.
%      %\riker runs \cmd{as}, \cmd{cc}, and \cmd{collect2} less often than \cmake.
%      %\riker runs \cmd{cc1} more than the default build system because it builds files in \file{src/common} multiple times.
%      \label{fig:redis-count}
%    }
%  \end{center}
%\end{figure}


==> riker-case-study.tex <==
As a final case study, we build \riker using a \rikerfile.
We compare this build to \riker's default build, which uses \make.
\riker is written in C++ and uses templates extensively, so build times can be quite long.
Building \riker and its dependencies compiles approximately 60,000 lines of source code (not including system includes or the standard library).
The complete \rikerfile we use to build \riker is included below:

\begin{lstlisting}[style=rikerfile]
#!/bin/sh
CFLAGS="..."
CXXFLAGS="$CFLAGS --std=c++17"
clang $CFLAGS -fPIC -shared -o libblake3.so |\Suppressnumber|
  deps/blake3/c/blake3.c ... |\Reactivatenumber|
clang++ $CXXFLAGS -o rkr src/*/*.cc |\Suppressnumber|
  -L. -lblake3 -lstdc++fs -lfmt |\Reactivatenumber|
clang $CFLAGS -o rkr-launch launch/launch.c
\end{lstlisting}

This \rikerfile builds the \blake dependency, the main \riker program, and the small \cmd{rkr-launch} program that \riker uses to bootstrap each build.
Unlike \blake, \cliEleven and \cereal do not need an extra command.
The full \rikerfile is 482 bytes, compared to 1624 bytes for \riker's \Makefile.
\riker's \Makefile makes extensive use of wildcards, pattern substitution, and compiler-assisted dependency generation to concisely specify an incremental build, but total size is nearly four times that of the equivalent \rikerfile.
Including the compiler-generated \file{.d} files, the \Makefile grows another 58KB.

\begin{figure}[t]
  \begin{center}
    \includegraphics{graphs/riker}
    \caption{
      Command counts and runtimes for 100 incremental builds of \riker.
      %\riker and its default \make build system perform virtually identical work, despite \make having a significantly more detailed specification.
      \riker runs 16\% fewer commands than \make.
      Building with \riker is only 6\% slower than \make.
      \label{fig:riker}
    }
  \end{center}
\end{figure}

Figure~\ref{fig:riker} shows the result of building \riker using this \rikerfile and its default \make build over the last 100 commits shortly before this paper was submitted.
\riker and \make perform nearly identical work, despite the significant differences in their  specifications.
\riker runs 16\% fewer commands than \make and takes just 6\% longer to build the entire sequence of 100 commits.
\riker generates a 5.7MB trace and caches 42 files totaling 10.3MB during this build.
The executable built by \riker passes all 114 tests in our test suite.

For this benchmark, command counts are almost identical because \clang does not invoke separate compilation and assembly commands.
Instead, the \cmd{clang -cc1} command uses an integrated assembler to directly emit \file{.o} files.
The lower overhead when building \riker may be partly due to the smaller number of commands launched during the build, but C++ compilation is also more computationally-intensive than in the other benchmarks so system call tracing is less of a bottleneck.



==> xz-case-study.tex <==
The \cmd{xz} project includes command-line compression and decompression tools, along with \cmd{liblzma}, which comprises roughly 21,000 lines of C source.
% DWB: This is wordy and seems to just invite attack... replaced with the sentence below.
% There are two build systems distributed with \cmd{xz};
% one that uses the standard autotools, \cmd{configure}, and \make build process, and a newer build process that uses \cmake.
% We use the \cmake build as a point of comparison, as this build system makes it easier to discover the intended build process than the autotools build.
We use \cmd{xz}'s \cmake build as a point of comparison.
The complete \rikerfile for \cmd{xz} is included below.

\begin{lstlisting}[style=rikerfile]
#!/bin/sh
CFLAGS='...'
LIBFLAGS='-fPIC -shared ...'
cc $CFLAGS $LIBFLAGS -o liblzma.so.5.3.1 |\Suppressnumber|
   src/common/*.c src/liblzma/*/*.c |\label{line:liblzma-wildcard}\Reactivatenumber|
ln liblzma.so.5.3.1 liblzma.so
ln liblzma.so.5 liblzma.so
cc $CFLAGS -o xz src/common/*.c src/xz/*.c |\label{line:xz-wildcard}\Suppressnumber|
   -L. -llzma |\Reactivatenumber|
cc $CFLAGS -o xzdec src/common/*.c |\label{line:xzdec-wildcard}\Suppressnumber|
   src/xzdec/*.c -L. -llzma |\Reactivatenumber|
\end{lstlisting}

Lines~\ref{line:liblzma-wildcard}, \ref{line:xz-wildcard}, and \ref{line:xzdec-wildcard} build the three targets with a single compiler invocation for each.
The only other change required to build \cmd{xz} with \riker was to rename five unused source files so they are not matched by the wildcard \file{src/liblzma/*/*.c}.
The entire \rikerfile for \cmd{xz} is 1620 bytes long, whereas the relevant portion of \cmd{xz}'s \file{CMakeLists.txt} file is nearly 8KB.

\begin{figure}[t]
  \begin{center}
    \includegraphics{graphs/xz}
    \caption{
      Build command counts and runtimes for incremental builds over 100 revisions of \cmd{xz}.
      \riker runs 59\% fewer commands than \cmake during incremental builds.
      \riker's build times are $3.53\times$ slower, but just $1.87\times$ for builds that run at least 10\% of commands.
      \label{fig:xz}
    }
  \end{center}
\end{figure}

Figure~\ref{fig:xz} shows the results of building \cmd{xz} using the provided \cmake build system and \riker over the 100 commits leading up to the latest release (version 5.2.5) of \cmd{xz}.
The upper plot shows the total number of commands run during the build at each commit.
The first commit is a full build, but every other commit invokes an incremental build.
\riker consistently runs fewer commands that \cmd{xz}'s \cmake builds, approximately to 41\% of \cmake's total.
% The targets built by \riker pass all tests provided with \cmd{xz}.

\begin{figure}[t]
  \begin{center}
    \includegraphics{graphs/xz.count}
    \caption{
      The number of times a subset of commands executed while building \cmd{xz}.
      \riker runs \cmd{as}, \cmd{cc}, and \cmd{collect2} less often than \cmake.
      \riker runs \cmd{cc1} more than the default build system because it builds files in \file{src/common} multiple times.
      % TODO: sort bars in ascending order if there's time
      \label{fig:xz-count}
    }
  \end{center}
\end{figure}

Figure~\ref{fig:xz-count} compares execution counts for the most common build commands.
The largest difference between the two builds is \cmd{cc};
because \cmd{cc} is a compiler driver, it is only responsible for launching \cmd{cc1} and \cmd{as}.
\riker only runs \cmd{cc1} during the first build.
On later builds \riker runs \cmd{cc1} and \cmd{as} directly.
\riker frequently skips runs of \cmd{as} because many commits make changes to \file{.c} and \file{.h} files that do not change the generated assembly.
This occurs when a commit only modifies a comment, or more commonly, when a change is confined to function declarations or preprocessor constants in \file{.h} files.
% Only the \file{.c} files that use these functions or constants are affected by the change.
Nevertheless, \riker must rerun \cmd{cc1} in these cases to discover inconsequential changes because \riker has no special understanding of C or any other programming language.
Much like \cmd{cc}, the \cmd{collect2} command runs only during the first build.
Only \cmd{ld} has to be rerun for new or changed \cmd{.o} files.

The one command that \riker runs more often than \cmake is \cmd{cc1}.
This can happen when \cmd{xz}'s build system is missing a dependency, but in this case it is due to the way the \rikerfile was written.
All three targets in this file---\cmd{xz}, \cmd{xzdec}, and \cmd{liblzma.so}---recompile the files in \file{src/common}.
Each time one of these files is modified, \riker runs \cmd{cc1} three times.

The lower plot in Figure~\ref{fig:xz} shows the runtime for the build at each commit.
While \riker runs fewer commands than \cmake, and its mean build time is $3.53\times$ higher, this number is strongly skewed by the higher cost of a no-change build with \riker.
Although the \cmake build system can perform these builds in microseconds, \riker's runtime is still well under a second, which is barely perceptible.
For more substantial changes, like commits that cause at least 10\% of the full build commands to run, \riker's overhead is only $1.87\times$.

This build exercises worst-case performance for \riker;
building \cmd{xz} invokes hundreds of short-lived commands, each of which incurs additional startup overhead in \riker as compared to \cmake.
Nevertheless, \riker's median build time is 0.6 seconds, and never exceeds 8.8 seconds for any commit.
\cmake has a median of 0.07 seconds, with a maximum of 4.4 seconds.
\riker runs far fewer commands than \cmake, so reductions in tracing overhead should significantly improve performance.
\riker's trace and file cache overheads are also modest;
\riker's trace is at most 25MB after each build, and the cache includes 191 files with a total size of 2.1MB.

% Probably not needed: revising the Rikerfile so it only compiles files in src/common/ once saves another 10%. It makes the Rikerfile uglier though.
